End-to-end Multiple Instance Learning with Gradient Accumulation

Being able to learn on weakly labeled data, and provide interpretability, are two of the main reasons why attention-based deep multiple instance learning (ABMIL) methods have become particularly popular for classification of histopathological images. Such image data usually come in the form of gigapixel-sized whole-slide-images (WSI) that are cropped into smaller patches (instances). However, the sheer size of the data makes training of ABMIL models challenging. All the instances from one WSI cannot be processed at once by conventional GPUs. Existing solutions compromise training by relying on pre-trained models, strategic sampling or selection of instances, or self-supervised learning. We propose a training strategy based on gradient accumulation that enables direct end-to-end training of ABMIL models without being limited by GPU memory. We conduct experiments on both QMNIST and Imagenette to investigate the performance and training time, and compare with the conventional memory-expensive baseline and a recent sampled-based approach. This memory-efficient approach, although slower, reaches performance indistinguishable from the memory-expensive baseline.

==> baackup.tex <==

\section*{Acknowledgements}
To my dearest friends, Håkan and Gupa, 


 

\section{Results}

We conduct experiments on datasets with 50, 100 and 300 train bags and 100, 300, 500, 800 instances per bag for both QMNIST-bags and Imagenette-bags. The number of test bags is equal to 60 for both considered datasets.
All the experiments are repeated 3 times with resampling the instances for bags.

\subsection{QMNIST-bags}

The number of validation bags is set to 30.
Positive bags of all the QMNIST-bags datasets contain 5\% of key instances per bag. Images are resized to $84\!\times\!84$ pixels during algorithms implementation and normalized by mean, std of QMNIST. 

Accuracy, AUC and time for training the models on QMNIST-bags are presented in Fig.~\ref{fig:QMNIST_performance}. 
Original ABMIL implementation and ABMIL with gradient accumulation with batch size equal to the number of instances per bag demonstrate the same accuracy at the bag level and AUC at the instance level, however, implementation of ABMIL with gradient accumulation is more time consuming, nonetheless, the difference is less than the order of magnitude.



\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[][50 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_bagLevel_0050_0005.pdf}}
 \quad
    \subfloat[][100 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_bagLevel_0100_0005.pdf}}
 \quad
    \subfloat[][300 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_bagLevel_0300_0005.pdf}}\quad\newline
  \subfloat[][50 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_insLevel_0050_0005.pdf}}
  \quad
  \subfloat[][100 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_insLevel_0100_0005.pdf}}
  \quad
 \subfloat[][300 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_insLevel_0300_0005.pdf}}\quad
  \subfloat[][50 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_time_0050_0005.pdf}}
  \quad
  \subfloat[][100 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_time_0100_0005.pdf}}
  \quad
 \subfloat[][300 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/QMNIST_time_0300_0005.pdf}}\quad
\caption{
Average (over 3 repetitions) test set performance for original ABMIL and ABMIL with gradient accumulation on QMNIST-bags 
(larger is better):
\textbf{Top:} Accuracy at the bag level. \textbf{Middle:} AUC at the instance level.
\textbf{Bottom:} Time for training. 
Error bars correspond to standard deviation over 3 repetitions. 
}
\label{fig:QMNIST_performance}
% \vspace{-3.5mm}
\end{figure*}


\subsection{Imagenette-bags}

The number of validation bags is set to 60.
Positive bags of all the QMNIST-bags datasets contain 30\% of key instances per bag. Images are normalized by mean, std of Imagenette.

% 3 repetitions only for 50train bags
\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[][50 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_bagLevel_50train_bags_.pdf}}
 \quad
    \subfloat[][100 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_bagLevel_100train_bags_.pdf}}
 \quad
    \subfloat[][300 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_bagLevel_300train_bags_.pdf}}\quad\newline
  \subfloat[][50 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_instanceLevel_50train_bags_.pdf}}
  \quad
  \subfloat[][100 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_instanceLevel_100train_bags_.pdf}}
  \quad
 \subfloat[][300 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_instanceLevel_300train_bags_.pdf}}\quad
  \subfloat[][50 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_time_50train_bags_.pdf}}
  \quad
  \subfloat[][100 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_time_100train_bags_.pdf}}
  \quad
 \subfloat[][300 train bags]{\includegraphics[width=0.3\textwidth,trim={1mm 2mm 1mm 2mm},clip]{./illustrations/Imagenette_time_300train_bags_.pdf}}\quad
\caption{
Average (over 3 repetitions) test set performance for original ABMIL and ABMIL with gradient accumulation on Imagenette-bags 
(larger is better):
\textbf{Top:} Accuracy at the bag level. \textbf{Middle:} AUC at the instance level.
\textbf{Bottom:} Time for training. 
Error bars correspond to standard deviation over 3 repetitions. 
}
\label{fig:Imagenette_performance}
% \vspace{-3.5mm}
\end{figure*}

